Guiding Neural Entity Alignment with Compatibility

Entity Alignment (EA) aims to find equivalent entities between two Knowledge Graphs (KGs). While numerous neural EA models have been devised, they are mainly learned using labelled data only. In this work, we argue that different entities within one KG should have compatible counterparts in the other KG due to the potential dependencies among the entities. Making compatible predictions thus should be one of the goals of training an EA model along with fitting the labelled data: this aspect however is neglected in current methods. To power neural EA models with compatibility, we devise a training framework by addressing three problems: (1) how to measure the compatibility of an EA model; (2) how to inject the property of being compatible into an EA model; (3) how to optimise parameters of the compatibility model. Extensive experiments on widely-used datasets demonstrate the advantages of integrating compatibility within EA models. In fact, state-of-the-art neural EA models trained within our framework using just 5\% of the labelled data can achieve comparable effectiveness with supervised training using 20\% of the labelled data.

==> sections/method.tex <==



\section{The \textsf{EMEA} Framework}


\subsection{Overview}
% describe the two modules, their roles in EMEA
%As shown in Fig.~\ref{fig:overview} (a), 


\textsf{EMEA} consists of two modules as shown in Fig.~\ref{fig:two_modules}.
%
The neural module is used to predict the probabilities of the candidate counterparts $q_\theta(y_v | x_v)$ of each unmatched entity $v$ based on its local features $x_v$ in an end-to-end manner. 
%
Meanwhile, the joint distribution module $p_\phi(y_L, y_U)$ is designed to measure the compatibility of a set of labels $y_L \cup y_U$, among which $y_U$ is predicted by the neural model. The dependencies of different labels are exploited here while the entity features are not.
The joint distribution model is based on Conditional Random Fields (CRF), in which the reasoning rules are used to construct its feature functions. Assignments of $y_L \cup y_U$ with higher compatibility with respect to these rules are more likely to have a higher joint probability. 

\noindent
We intend to have a well-trained joint distribution module to guide the training of the neural model.
However, as mentioned in Sec.~\ref{sec:em_background}, the joint distribution module is challenging to optimise because its parameters depend on the latent labels.
To solve this problem, we apply variational EM framework to marry the two modules together through a joint optimisation process, as shown in Fig.~\ref{fig:em_proc}.
The neural module is initially trained with labelled data, while the joint probability module performs random initialisation.
In the M-step, we sample the label of each unlabelled entity from current neural module and update $p_\phi$ with $\hat{y}_L$ and $\hat{y}_U \sim q_\theta (y_U)$.
In the E-step, the joint distribution module derives more compatible predictions $\hat{y}_U$ than the current neural model and uses $\hat{y}_L \cup \hat{y}_U$ to renew the neural module. 


% \vspace{-8pt}
\subsection{Measure Self-consistency}

\subsubsection{CRF-based Probabilistic Model of Labels}

We model the probability distribution over a set of labels $y_L \cup y_U$ with CRF~\cite{DBLP:journals/ftml/SuttonM12},\footnote{The effects among entities are not directed and thus we choose undirected graphical models rather than directed ones like Bayesian Networks. Then, the rules only exploit the dependencies between labels without involving features. So we choose CRF.} which is a graphical model and can be factorised by a product of \textit{local functions} (or called compatibility functions) that depend on a few variables. 
Given a collection of subsets $y_A \subset y_V $ where $A$ is a small entity set, the joint distribution can be written as 

\vspace{-8pt}
\begin{equation}
    p(y_V) = \frac{1}{Z} \prod_A \phi_A (y_{A})
    \label{eq:p_v}
\end{equation}

\vspace{-4pt}
\begin{equation}
    Z = \sum_{y'_V} \prod_A \phi_A(y'_{A})
    \label{eq:p_z}
\end{equation}

\noindent
Here, $\phi_A(y_A)$ is a local function defined on a subset $y_A$ and will be further explained below.
$Z$ is a normalisation factor. 

% The parameters $w_k$ are the variables of $Z$. When $w_k$ are fixed, $Z$ becomes a constant.


\begin{figure}
    \begin{subfigure}[b]{0.25\textwidth}
        \includegraphics[width=4cm]{images/factor_graph_paris.pdf}
        \caption{For PARIS rule}
        \label{fig:factor_graph_paris}
    \end{subfigure}%
    \begin{subfigure}[b]{0.25\textwidth}
        \includegraphics[width=3.8cm]{images/factor_graph_one2one.pdf}
        \caption{For one-to-one restriction}
        \label{fig:factor_graph_onetoone}
    \end{subfigure}
    \vspace{-20pt}
    \caption{Examples of building factor graphs.}
    % \vspace{-12pt}
\end{figure}


\subsubsection{Local Functions Based on Reasoning Rules}~\label{sec:local_functions}
In general, given a rule, we first build a collection of \textit{factor graphs}. Each factor graph consists of a small set of labels $y_A$ that we check the rule on.
Then, if (or to what extent) a certain rule $k$ is met is expressed with one \textit{feature function} $g_k(y_A)$.
Considering different rules can be defined on the same factor graph, we derive the local function defined on a set of labels $y_A$ with the form below, where $w_k$ are parameters.
\begin{equation}
	\phi_A (Y_{A}) = \exp\left(  \sum_k w_k g_k(Y_{A}) \right)
    \label{eq:local_function}
\end{equation}
%
Note each local function is defined on a certain factor graph and different local functions can be combined through Eq.~\ref{eq:p_v}. 


Next, to show how we go from rules to local functions concretely in the scenario of EA, we construct local functions based on two different types of rules as examples.

\paragraph{PARIS rule}

% The PARIS rule is a sufficient and necessary rule, whose effectiveness has been empirically verified to be effective by existing works~\cite{DBLP:journals/pvldb/SuchanekAS11,DBLP:journals/pvldb/SunZHWCAL20,DBLP:journals/tkde/ZhaoZTWS22}.
PARIS rule is used to check the label compatibility of each entity with its neighbours in the KG. To construct the factor graphs, as shown in Fig.~\ref{fig:factor_graph_paris}, at each entity we create a factor graph which connects the anchor entity with its adjacent entities according to the KG structure.
Then, we get the corresponding feature function $g(y_{A_v})=\Pr(v \equiv y_v)$ with Eq.~\ref{rule:paris_prob}.


\paragraph{One-to-one restriction.}\label{sec:one2one}
Instead of checking if each entity's label is different from all other entities, we only check few entities with most similar embeddings (derived from the neural model) with it as approximation.
%
As shown in Fig.~\ref{fig:factor_graph_onetoone}, over each entity, we create a factor graph containing the anchor entity and its nearest $N$ neighbours in embedding space.
The corresponding feature function indicates \textit{if the anchor entity has a unique label} (denoted as \textit{One2one}).
%
In addition, because one-to-one restriction is necessary but not sufficient for EA,~\footnote{Under the one-to-one assumption, good EA results should meet this restriction, but EA results with higher one-to-one compatibility are not necessarily better in effectiveness.} we introduce an assistant rule: \textit{each entity's label equals the prediction of the neural model} (denoted as \textit{EqNeu}). Each factor graph simply contains one anchor entity. 

It should be noticed that the PARIS rule is used as the primary reasoning rule of \textsf{EMEA} for its excellent performance. 
We introduce one-to-one restriction because it is very different from PARIS rule in terms of sufficiency and the construction of factor graph. We will use it to explore the generality of \textsf{EMEA} and the effect of different types of rules in \textsf{EMEA} in experiments.


\subsubsection{Simplified Conditional Probability.}
In the CRF-based distribution, an entity $v$ is only involved in a few local functions. Thus, we can simplify the conditional distribution $p(y_v|y_{V\setminus\{v\}})$ to be $p(y_v|y_{MB(v)})$ as in Eq.~\ref{eq:conditional_prob}, where $MB(v)=\bigcup_{v \in A} A \setminus\{v\}$ is the Markov blanket. 
% With this conditional distribution, we can further get the marginal distribution $p(y_e)$ as in Eq.~\ref{eq:marginal_prob}. 
This conditional probability is used to update the two modules in the following sections. The factor graphs make some computations (e.g., in Eq.~\ref{eq:objective_pl_phi} and Eq.~\ref{eq:coordinate_update}) much easier since only a small number of entities $MB(v)$ are involved in computing the expectation.

% \vspace{-8pt}
% \begin{equation}
%     \begin{split}
%         p_\phi(y_v | y_{V \setminus \{v\}}) & = p_\phi(y_v | y_{MB(v)}) \\
%         & = \frac{\prod_{A | v \in A}{\phi_A(y_{A})} }{\sum_{v' \in V'} \prod_{A | v \in A}\{\phi_A(y_{A}) | y_v=v' \} } 
%     \end{split}
%     \label{eq:conditional_prob}
% \end{equation}


\vspace{-8pt}
\begin{multline}
    p_\phi(y_v | y_{V \setminus \{v\}}) \\
    = \frac{\prod_{A|v \in A} \phi_A(y_A) \prod_{A|v \notin A} \phi_A(y_A)}{\sum_{v' \in V'} \prod_{A|v \in A} \phi_A(y_v=v', y_{A\setminus \{v\}}) \prod_{A|v \notin A} \phi_A(y_A)} \\
        = \frac{\prod_{A | v \in A}{\phi_A(y_{A})} }{\sum_{v' \in V'} \prod_{A | v \in A} \phi_A(y_v=v', y_{A \setminus \{v\}}) } 
        = p_\phi(y_v | y_{MB(v)}) 
        \label{eq:conditional_prob}
\end{multline}






\subsection{Train Neural Model with Self-consistency}\label{sec:estep}

In the E-step, we update $q_\theta$ to maximise the ELBO $Q(p_\phi, q_\theta)$ (Eq.~\ref{eq:em_objective}) with current $p_\phi$ fixed. % and the updated $q_\theta(y_U|x_U)$ can be used as approximation of $p_\phi(y_U|x_U, y_L)$.
By re-writing $Q(p_\phi, q_\theta)$ as in Eq.~\ref{eq:em_kl}, maximising $Q(p_\phi, q_\theta)$ is equivalent to decreasing the KL-divergence between $q_\theta(y_U)$ and $p_\phi(y_L, y_U)$ ($y_L$ is known), i.e. making them closer in distribution. Assuming the current $p_\phi$ reflects the compatibility of labels, the updated $q_\theta$ can make more compatible predictions.

\vspace{-8pt}
\begin{equation}
    \begin{split}
        Q(p_\phi, q_\theta) & = \mathbb{E}_{q_\theta(y_U)} [ \log p_\phi(y_L, y_U) -  \log q_{\theta}(y_U) ] \\
        & = - \mathbb{E}_{q_\theta(y_U)} \left[ \log \frac{q_{\theta}(y_U)}{p_\phi(y_L, y_U)} \right] 
         = - KL(q_{\theta}(y_U) || p_\phi(y_L, y_U))
    \end{split}
    \label{eq:em_kl}
\end{equation}

%
It takes two stages to update $q_\theta$. 
In the first stage, we derive a better $q^*(y_U)$ than the current $q_\theta(y_U)$ with coordinate ascent mean field variational inference~\cite{DBLP:journals/corr/BleiKM16}.
Specifically, we use current $q_\theta(y_U)$ as the starting point of $q(y_U)$. Then, in each iteration, we select one or a block of entities $v$ to update their probabilities $q(y_v)$, as in Eq.~\ref{eq:coordinate_update}. The probability $q(y_v)$ of each entity $v$ is updated in turn until $q(y_U)$ converges.
Eventually, this coordinate ascent procedure converges to a local maximum $q^*(y_U)$.

\vspace{-8pt}
\begin{equation}
    q^*(y_v) \propto  \exp \left( \mathbb{E}_{q_\theta(y_{MB(v)})} [\log p_\phi (y_v | {y}_{MB(v)})] \right) 
    \label{eq:coordinate_update}
\end{equation}

\noindent
We take three measures to make computing $q^*(y_U)$ more efficient:

\hangpar
\textbf{(I)} To reduce computation cost, we only sample one alignment $\hat{y}_U$ to estimate the expectation in Eq.~\ref{eq:coordinate_update}. For an unlabelled entity $v$, we sample $\hat{y}_v=\mathrm{argmax}_{v' \in V'} q(y_v=v')$. For labelled entities, we use their ground-truth labels.

\hangpar
\textbf{(II)} When computing Eq.~\ref{eq:coordinate_update} for a specific entity, we meet a similar challenge as in Sec.~\ref{sec:update_joint}: it is too time-consuming to consider all entities $v' \in V'$ in the target KG as candidates to compute $q(y_v=v')$. Therefore, we use a similar process: only perform this for the top $K$ candidate counterparts of each entity. As a result, the obtained $q(y_v)$ is not an exact local maximum.

\hangpar
\textbf{(III)} We update $q(y_v)$ for all entities in a single iteration of coordinate ascent to avoid the potential error propagation of approximated $q(y_v)$ in step II. Eventually, we get $q^*(y_v)$ as below

\begin{equation}
    q^*(y_v) \propto p_\phi (y_v | \hat{y}_{MB(v)}), v \in U
\end{equation}

\noindent
In the second stage, we treat $q^*(y_U)$ as a target to help update the neural model. Specifically, we sample $\hat{y}_v = \mathrm{argmax}(q^*(y_v))$ for the unlabelled entities $U$. These sampled data are combined with the labelled data as training data to continue training the neural model.








\subsection{Mapping Neural Similarity to Probability}% for Neural Model}
\textsf{EMEA} requires the neural module to output the probabilities of candidate counterparts for each entity. However, most neural EA models only output similarities between each entity and the candidates. Therefore, we introduce a separate model to normalise the similarities to probabilities. 
%
% Simply modifying the model structure by using one softmax layer as output and training the model with cross entropy loss has been shown to worsen the effectiveness~\cite{DBLP:conf/www/MaoWWL21}.
% Therefore, we exploit a separate model to map the similarities of neural EA models to probabilities. 
%
Given an entity $v$ and its similarities $S_{v,v'}$ to all entities $v'$ in the target KG, we use $S_{v,v'}$ and $\delta_{v,v'}=\max(S_{v,:})-S_{v,v'}$ as the features of entity pair $(v,v')$. These features are combined linearly and fed into a softmax function with a temperature factor $\tau$, as shown in Eq.~\ref{eq:simtoprob_1} and~\ref{eq:simtoprob_2}. The learnable parameters include $a_1,a_2,b$ and $\tau$. Cross-entropy loss is chosen for optimisation and the model is trained with labelled data.
\begin{equation}
    \hat{S}_{v,v'} = a_1 * S_{v,v'} + a_2 * \delta_{v,v'} + b
    \label{eq:simtoprob_1}
\end{equation}
\begin{equation}
    q_\theta(y_v=v') = \frac{\exp(\hat{S}_{v,v'}/\tau)}{ \mathrm{sum}\left( \exp(\hat{S}_{v,:}/\tau) \right)  }
    \label{eq:simtoprob_2}
\end{equation}


\subsection{Optimization based on EM}\label{sec:update_joint}

When updating $p_\phi$, we assume the correct distribution of latent variables is the current $q_\theta(y_U)$ and keep it fixed. 
The optimisation objective is to maximise Eq.~\ref{eq:em_objective} with respect to $\phi$, which is equivalent to maximising Eq.~\ref{eq:objective_phi} as the second item in Eq.~\ref{eq:em_objective} is irrelevant to the parameter $\phi$. 
\begin{equation}
    l(\phi) = \mathbb{E}_{q_\theta(y_U)} [\log p_\phi (y_L, y_U)]
    \label{eq:objective_phi}
\end{equation}
\noindent
In practice, we take four steps to address optimisation challenges:

\hangpar
\textbf{(I)} Computing the joint probability $p_\phi(y_L, y_U)$ is complex because it involves normalisation (refer to Eq.~\ref{eq:p_v} and \ref{eq:p_z}). We exploit its pseudo-likelihood function~\cite{besag1975statistical} as shown below.

\begin{equation}
    p(y_L, y_U) \approx \prod_{v \in L \cup U} p(y_v | y_{V \setminus \{v\}})
    \label{eq:pseudo_likelihood}
\end{equation}
\noindent
Then, the objective function can be approximated as in Eq.~\ref{eq:objective_pl_phi}, which makes the optimisation computationally simpler. 

\vspace{-8pt}
\begin{equation}
    \begin{split}
        l(\phi) \approx
        l_{PL}(\phi) & = \mathbb{E}_{q_\theta(y_U)} [\sum_{v \in L \cup U} \log p_\phi ({y}_v | {y}_{V \setminus \{v\}})] \\
        & = \mathbb{E}_{q_\theta(y_U)} [ \sum_{v \in L \cup U} \log p_\phi ({y}_v | {y}_{MB(v)}) ]
    \end{split}
    \label{eq:objective_pl_phi}
\end{equation}

\hangpar
\textbf{(II)} The expectation in Eq.~\ref{eq:objective_pl_phi} can be estimated by drawing samples from $q_\theta(y_U)$. We only choose one sample. Specifically, we sample $\hat{y}_v = \mathrm{argmax}_{v' \in V'} q_\theta(y_v=v')$ if $v \in U$, otherwise $\hat{y}_v$ is the ground-truth label. In this way, Eq.~\ref{eq:objective_pl_phi} is further simplified as 
\begin{equation}
    l_{PL}(\phi) \simeq \sum_{v \in L \cup U} \log p_\phi (\hat{y}_v | \hat{y}_{MB(v)})
    \label{eq:sample_pl}
\end{equation}

\hangpar
\textbf{(III)} The computation of $p_\phi(y_v|y_{MB(v)})$, as shown in Eq.~\ref{eq:conditional_prob}, involves all entities $v' \in V'$ in the target KG as possible candidate counterparts in the denominator.
This is very time-consuming since there is always a large amount of entities in the target KG. This makes EA different from common classification problems which do not have as many categories to classify. We address this problem by only selecting the top $K$ candidates $C_v$ from the target KG for each entity $v$ according to the current neural EA model. Formally: 
\begin{equation}
    \gamma = \sum_{v' \in C_v} q_\theta(y_v=v')
\end{equation}
\begin{equation}
    \tilde{p}_\phi(y_v=v' | y_{MB(v)}) \approx 
    \begin{cases}
         \gamma \frac{\prod_{A | v \in A}  \phi_A (y_v = v', y_{A \setminus \{v\}}) }{\sum_{v'_j \in C_v}\prod_{A | v \in A}  \phi_A (y_v = v'_j, y_{A \setminus \{ v \}}) } , v' \in C_v \\
        q_\theta (y_v = v'), v' \notin C_v
    \end{cases}
\end{equation}

\hangpar
\textbf{(IV)} Finally, we only sum up $\log p_\phi (\hat{y}_v | \hat{y}_{MB(v)})$ over labelled entities instead of all entities in Eq.~\ref{eq:sample_pl} because we find it more effective in practice. Note that the unlabelled entities are still involved in computing $\log p_\phi (\hat{y}_v | \hat{y}_{MB(v)}), v \in L$. Eventually, the final objective function to maximise is:
\begin{equation}
    O_\phi = \sum_{v \in L} \log \tilde{p}_\phi (\hat{y}_v | \hat{y}_{MB(v)})
    \label{eq:objective_phi_sampling}
\end{equation}








==> sections/only_equations.tex <==

\section{Draft - ONLY Equations}


\begin{table}
    \centering
    \begin{tabular}{c|c}
        \hline
        Symbols & Comment \\
        \hline
        $\mathcal{G}$& KG \\ 
        $\mathcal{G}, \mathcal{G}'$ & source, target KG \\
        $ E, E'$ & Source, target entity sets \\
        $L, U \subset E$ & Labelled and unlabelled entities \\
        $i \in E$ & the $i$-th source entity \\
        $y_i$ &  counterpart of the $i$-th entity \\
        $y_E, y_L, y_U$ & collective counterparts of entity set $E, L, U$ \\
        $q_\theta (y_i)$ &  label prob of neural module \\ 
        $p_\phi (y_E)$ & joint prob  or self-consistency \\
        $F$ & Entities in factor graph \\
        \hline
    \end{tabular}
\end{table}

% self-consistency -> local compatibilities.

\subsection{Self-consistency}

% We decompose the overall compatibility of $y_E$ into the local compatibilities $y_F$ of some entity subsets $F \in \mathbb{F}$.
% The factor graphs are built according to the requirement of compatibility checking.

Build many subsets $\mathcal{F} = \{ F_i \subset E \}$ to check.

Indicator function of rule $k$:
$$g_k(y_F) \in R$$

% local compatibility
% The compatibility function, i.e. local function of a certain factor graph $\mathcal{F}$ formed by a set of entities $F$ is defined as

local compatibility:
$$ \Phi (y_F) = \exp \left(\sum_k w_k * g_k(y_F) + b \right)$$

% Multiple rules can be defined on the same factor graph.

% joint prob of a certain set of predictions
% The joint prob of all counterparts -- overall self-consistency -- is defined as
overall compatibility or self-consistency:
$$ p(y_E) = \frac{1}{Z} \prod_{F \in \mathcal{F}} \Phi (y_F) $$

$$ Z = \sum_{y_U \in E^{|U|}} \prod_{F \in \mathcal{F}} \Phi(y_F) $$

% problem
$Z$ is intractable because it involves integral over $y_U \in E^{|U|}$, which is a very large space.

Simplification of conditional prob

Introduce concept Markov Blanket:
$\mathcal{F}^i = \{F_j | i \in F_j\}$


\begin{equation}
    \begin{split}
        p(y_i | y_{-i}, y_L) = \frac{p(y_L, y_U)}{p(y_{-i}, y_U)} = \frac{p(y_U, y_L)}{\sum_{e' \in E'} p(y_i=e', y_{-i}, y_L)} \\
        = \frac{\prod_{F \in \mathcal{F}^i} \Phi(y_F) \prod_{F \in \mathcal{F} \setminus \mathcal{F}^i} \Phi(y_F)}{\sum_{e' \in E'} \prod_{F \in \mathcal{F}^i} \Phi(y_F | y_i=e') \prod_{F \in \mathcal{F} \setminus \mathcal{F}^i} \Phi(y_F)} \\
        = \frac{\prod_{F \in \mathcal{F}^i} \Phi(y_F) }{\sum_{e' \in E'} \prod_{F \in \mathcal{F}^i} \Phi(y_F | y_i=e') }
        = p(y_i | y_{MB \setminus i})
    \end{split}
\end{equation}



\subsection{Power Neural EA with Self-consistency}
% joint prob -> self-consistency
Make $q(y_U)$ close to $p(y_U | y_L)$ 

% update neural EA model
% make $q(y_U)$, which can be written as $\prod_{e \in U} q_(y_e)$, close to $p(y_U|y_L)$.
To this end, we minimize 
\begin{equation}
    \begin{split}
        \mathrm{KL}(q(y_U) || p(y_U|y_L)) = \mathbb{E}_{q(y_U )} \log \frac{q(y_U)}{p(y_U|y_L)}   \\
        = \mathbb{E}_{q(y_U)} \log q(y_U)  - \mathbb{E}_{q(y_U)} \log p(y_U|y_L) \\
        = \mathbb{E}_{q(y_U)} \log q(y_U) - \mathbb{E}_{q(y_U)} \log p(y_U, y_L) \\ + \mathbb{E}_{q(y_U)} \log p(y_L) \\
        = -\left( \mathbb{E}_{q(y_U)} \log p(y_U, y_L) - \mathbb{E}_{q(y_U)} \log q(y_U) \right)  +  \log p(y_L) 
    \end{split}
\end{equation}
% the last item irrelevant to $y_U$. So it is a constant.

% To simplify computation, we choose to minimize $KL(q,p)$.

% It is not easy to optimize $KL(p||q)$ directly, so we optimize its 
Evidence Lower Bound (ELBO)
$$ L_\theta = \mathbb{E}_{q_\theta (y_U)} \log p(y_U, y_L) - \mathbb{E}_{q_\theta (y_U)} \log q_\theta (y_U) $$


% $$ \mathbb{E}_{q(y_U)} \log q(y_U) = \sum_{e \in U} \mathbb{E}_{q(y_e)} \log q(y_e) $$

neural model make independent predictions, so
$$q(y_U) = \prod_{i \in U} q(y_i) $$

to make the computation of the joint prob simpler, we use pseudolikelihood to approximate it.
$$ p(y_U, y_L) = p(y_L) \prod_{i \in U} p(y_{i} | y_{1:i-1}, y_L ) 
\approx p(y_L) \prod_{i \in U} p(y_i | y_{-i}, y_L )  $$

then, we can re-write the ELBO as 
\begin{equation}
    \begin{split}
         \log p(y_L) + \sum_{i \in U} \mathbb{E}_{q(y_i)} \left[ \mathbb{E}_{q({y_{-i}})}  \left[ \log p(y_i | y_{-i}, y_L) \right] - \log q(y_i) \right]
    \end{split}
\end{equation}


derive the coordinate ascent update for the latent variables
$$ q^*(y_i) \propto \exp \left(\mathbb{E}_{q(y_{-j})} [ \log p(y_i | y_{-i}, y_L) ] \right) $$

Here, 



\subsection{Optimization - EM}

optimize parameters $\phi$ of $p$ by maximizing the observed data

\begin{equation}
    \begin{split}
        \log p(y_L) = \log \sum_{y_U} p(y_L, y_U) 
    \end{split}
\end{equation}


because of the interdependency between $y_U$ and $\phi$, we use EM to do the optmization.

In E-step, we compute the expectation of $\log p(y_L, y_{U})$, i.e. $\mathbb{E}_{p(y_U|y_L)} \log p(y_L, y_U)$.
Here, we approximate $p(y_U|y_L)$ with $q(y_U)$. 
$$L_{\phi} = \mathbb{E}_{q(y_U)} [ \log p(y_L, y_U) ] $$

In M-step, we update $\phi$ to maximize $L_{\phi}$.


The whole EM process is described in Algo xxx.
























==> sections/preliminary.tex <==
\section{Preliminaries}


\subsection{Notions and Problem Definition}
%  \todo{why call the set of entities $V$? why not something easier to refer to, $E$? Or is this the common notation?}

% We denote a KG as $G=\left\langle V, R, T \right\rangle$, where $V$ is the entity set, $R$ is the relation set, and $T$ is the triple set.

One KG basically consists of entities and triples.
Given two KGs $G$ and $G'$ with entity sets $V$ and $V'$ respectively, the goal of EA is to match the source entities $v\in V$ with equivalent target entities $v'\in V'$, with an assumption that the mapping of entities is one-to-one.
%One-to-one mapping is assumed. %(i.e., each source entity can only match with a single target entity).
%
% We treat the source entities as data instances while target entities are categories.
For each source entity $v \in V$, we denote its feature variable as $x_v$ and label (equivalent entity in the target KG) variable as $y_v \in V'$. The features and labels of a set of entities $V$ is analogously denoted as $x_V$ and $y_V$.

In this work, we formulate EA as a semi-supervised problem.
That is, all entities $v\in V$ are given, but only the labels $y_L$ of a subset $L \subset V$ are observed. The labels $y_U$ of unlabelled source entities $U \subset V$ are treated as latent variables. Our goal is to produce a model that predicts $y_U$.

%
\textsf{EMEA} combines a neural module (with parameters $\theta$) that predicts the probability $q_\theta(y_v|x_V, y_L)$ of each possible label $y_v \in V'$ for each unmatched source entity $v \in U$, and a joint distribution module (with parameters $\phi$) that measures the joint probability $p_\phi(y_V|x_V)$ (i.e. $p_\phi(y_L, y_U|x_V)$) of a set of predictions.
The optimisation of the joint distribution module $p_\phi$ involves both observed and latent labels $y_L, y_U$ and thus has special challenges which will be further explained in Sec.\ref{sec:em_background}.
%
Considering the entity information in KGs and the labelled data are usually fixed, we remove $x_V$ and $y_L$ from the condition variables for simplicity 
(e.g., $q_\theta(y_v|x_V, y_L)$ to $q_\theta(y_v)$ and $p_\phi(y_V|x_V)$ to $p_\phi(y_V)$)
when there is no ambiguity.
The assignment to $y_v$ is denoted as $\hat{y}_v$.



% \vspace{-4pt}
\subsection{Reasoning-based EA Methods}\label{sec:paris}

The fundamental idea of reasoning-based EA methods is to infer the label of one entity according to the labels of its neighbouring entities.
In this work, we utilise one rule from \textit{PARIS}~\cite{DBLP:journals/pvldb/SuchanekAS11} defined by Suchanek et al. because it is a representative of reasoning-based methods.
Intuitively, this rule can be described as: 
\begin{myquote}{8pt}
Given a pair of entities $v_1$ and $v'_1$ from two KGs, if there exists two triples $r(v_1,v_2)$, $r(v'_1,v'_2)$ whose relation $r$ has high inverse functionality $fun^{-1}(r)$ and entities $v_2$ and $v'_2$ are equivalent, then $v_1$ and $v'_1$ have a high likelihood of being equivalent.~\footnote{A \textit{functional} relation can only have one object for a given subject. \textit{Functionality} is used to measure this property quantitatively. The inverse functionality of a relation is the functionality of its inverse  relation.}
\end{myquote}
Formally, this rule can be expressed as Eq.~\ref{rule:paris_positive_semantic}. Suchanek et al. further transformed this rule into a probabilistic form shown in Eq.~\ref{rule:paris_prob}. 
The rule described above require pre-aligned relations. To drop this restriction, Suchanek et al. applied statistical subsumption between relations to replace the pre-alignment of relations and re-wrote Eq.~\ref{rule:paris_prob} into a more complex form~\cite{DBLP:journals/pvldb/SuchanekAS11}.
The reasoning rule explained above has been exploited to achieve great success in some experimental settings~\cite{DBLP:journals/pvldb/SuchanekAS11,DBLP:journals/pvldb/SunZHWCAL20,DBLP:journals/tkde/ZhaoZTWS22}.

\vspace{-12pt}
\begin{equation}
    \begin{split}
        \exists~r, v_1, v'_1: & r(v_1,v_2) \wedge r(v'_1, v'_2) \wedge v_2 \equiv v'_2 \wedge fun^{-1}(r)~\text{is high}  \\ & \Longrightarrow v_1 \equiv v'_1 
    \end{split}
    \label{rule:paris_positive_semantic}
\end{equation}
\vspace{-8pt}

% \begin{equation}
%     \exists~r, y: r(x,y) \wedge fun(r)~\text{is high} \wedge (\forall r(x',y'): y \not\equiv y') \Longrightarrow x \not\equiv x' 
% \end{equation}
\vspace{-8pt}
\begin{equation}
    \Pr (v_1 \equiv v'_1) = 1 - \prod_{r(v_1,v_2), r(v'_1,v'_2)} \left(1 - \Pr (v_2 \equiv v'_2) \times fun^{-1}(r)\right)
    \label{rule:paris_prob}
\end{equation}
\vspace{-16pt}

% \begin{equation}
%     g(x \equiv x') =  \prod_{r(x,y)} \left( 1 - fun(r) \prod_{r(x', y')} (1- p(y \equiv y'))  \right) 
% \end{equation}

\noindent
%The reasoning rule explained above have been used as a sufficient and necessary condition and achieved great success under some experimental settings. However, there are also some other rules like one-to-one mapping restriction which are necessary but not sufficient, but are also very useful in error diagnosis of EA systems~\cite{DBLP:conf/semweb/Jimenez-RuizG11}.


% it has also been used for other purposes such as the diagnosis of errors in EA systems~\cite{DBLP:conf/semweb/Jimenez-RuizG11}.


\subsection{Neural EA Methods}

% Different from reasoning-based methods, neural EA methods focus on learning effective representations of entities for their matching and ignore the dependencies of labels.
Various neural EA models have been recently proposed~\cite{DBLP:journals/pvldb/SunZHWCAL20,DBLP:journals/tkde/ZhaoZTWS22,DBLP:conf/www/PeiYHZ19,DBLP:conf/www/ZhuWSZFD020,DBLP:conf/ijcai/HuangLYN20}. They generally work by encoding the local features of entities such as attributes and structure into vector representations (embeddings).
% Entities in the source and target KGs that share the highest similarity are matched (i.e., measured using the distance to each other in vector space with cosine similarity). 
For each source entity, the target entity that has the highest similarity (e.g., cosine similarity) with it in vector space is selected as its counterpart.
This process is formalised in Eq.~\ref{eq:neural_ea}, where $H$ and $H'$ represent the entity embedding matrices of the source and target KG respectively, and each row of them corresponds to the representation of a certain entity, $\mathrm{Enc}$ denotes KG encoder, and $S$ is a similarity matrix.
Neural models can be trained end-to-end with pre-aligned entity pairs.
% \vspace{-4pt}
\begin{equation}
    H = \mathrm{Enc}(G), H' = \mathrm{Enc}(G'), S=H \cdot {H'}^\top,
    \hat{y}_v = \mathrm{argmax}_{v'} S_{v,v'}
    \label{eq:neural_ea}
\end{equation}



\begin{figure*}[!t]
    \vspace{-8pt}
    \begin{subfigure}[b]{0.5\textwidth}
        \centering
        \includegraphics[width=6.5cm]{images/two_modules.pdf}
        \vspace{-8pt}
        \caption{Two modules.}
        \label{fig:two_modules}
    \end{subfigure}\hfill
    \begin{subfigure}[b]{0.5\textwidth}
        \centering
        \includegraphics[width=8cm]{images/overview2.pdf}
        \vspace{-8pt}
        \caption{EM process.}
        \label{fig:em_proc}
    \end{subfigure}
    \vspace{-20pt}
    \caption{Overview of the \textsf{EMEA} framework. (a) \textsf{EMEA} consists of two modules: one neural module for predicting correspondences end-to-end and one joint probability module for checking the compatibility of predicted correspondences. (b) The two modules are trained iteratively with variational EM.}
    \vspace{-8pt}
\end{figure*}


\vspace{-8pt}
\subsection{EM and Mean Field Variational Inference}\label{sec:em_background}
% \todo{optimize->optimise, minimize->minimise, etc.}

% \todo{I think this is unclear when you start talking about observed and unknown labels within the same model -- is this because \textsf{EMEA} is trained in a semi-supervised setting, therefore you need to have observed+unknown? Need to say why this challenge is required in the first place (i.e., the definitions in section 3.1).}

The joint distribution module $p_\phi(y_L, y_U)$ is critical in our framework. However, it is challenging to optimise the parameters $\phi$ of model $p_\phi(y_L, y_U)$ which involves both observed labels and unknown (latent) labels. The reason is the optimisation goal -- maximising the log likelihood of observed labels, i.e. $\log p_\phi(y_L)=\log \sum_{y_U} p_\phi(y_L, y_U)$ -- has an interdependency between the parameters $\phi$ and the unknown labels $y_U$. 
%
A solution to this challenge is the Expectation-Maximisation (EM) algorithm~\cite{dempster1977maximum}, which: (1) in the E-step, fixes the parameters and estimates the posterior of unknown labels $p_\phi(y_U|y_L)$; and (2) in the M-step, assumes the current posterior estimation $p_\phi(y_U|y_L)$ is correct and uses it to update the parameters. The iterative EM steps permit the parameters and posterior to converge.

% \todo{Again, saying \textit{why} you need $y_U$ and $y_L$ is necessary to say before you talk about the challenge itself.}
In the EM-algorithm,
another challenge occurs when inferring the posterior $p_\phi(y_U|y_L)$, which is needed by the E-step as mentioned above. It involves computing complex integration and is intractable if the space of $y_v$ is very large. To overcome this challenge, approximation methods of this posterior like loopy belief propagation~\cite{DBLP:conf/uai/MurphyWJ99} and mean field variational inference~\cite{DBLP:journals/ijon/Hogan02} have been proposed. 
In particular, mean field variational inference applies another distribution $q_\theta(y_U|y_L)$ ($\theta$ are parameters) that can be factorised into $\prod_{v \in U} q_\theta(y_v)$ to approximate $p_\phi(y_U|y_L)$.

Variational EM~\cite{DBLP:conf/icml/QuBT19,DBLP:conf/nips/Qu019}, which is a variant of the general EM algorithm~\cite{DBLP:books/sp/12/NealH98}, addresses these two challenges in a single framework.
With variational EM, we only need to optimise the evidence lower bound (ELBO) $Q(p_\phi, q_\theta)$ of $\log p_\phi(y_L|x_L)$ as in Eq.~\ref{eq:em_objective}. The equation holds when $q_\theta (y_U) = p_\phi (y_U|y_L)$. In the E-step, we fix $p_\phi$ and update $q_\theta$ to maximise $Q(p_\phi, q_\theta)$. In the M-step, we in turn assume $q_\theta$ is the true posterior, fix it and update $p_\phi$ to maximise $Q(p_\phi, q_\theta)$. 

\vspace{-8pt}
\begin{equation}
    \begin{split}
        \log p_\phi(y_L) & \geq Q(p_\phi, q_\theta) \\
        & = \mathbb{E}_{q_\theta(y_U)} [ \log p_\phi(y_L, y_U) -  \log q_{\theta}(y_U) ]
    \end{split}
    \label{eq:em_objective}
\end{equation}
\vspace{-16pt}





==> sections/tables/overall_iterative.tex <==
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
    \hline
    \multirow{2}{*}{Anno.} & \multirow{2}{*}{Method} &\multicolumn{3}{c|}{zh\_en}&\multicolumn{3}{c|}{fr\_en}&\multicolumn{3}{c|}{ja\_en}\\
     & & Hit@1&MRR&MR&Hit@1&MRR&MR&Hit@1&MRR&MR\\
    \hline
    \multirow{2}{*}{1\%} & RREA & 0.309&0.405&344.0&0.277&0.382&214.0&0.263&0.348&356.6\\
     & EMEA & \textbf{0.471}&\textbf{0.541}&\textbf{235.7}&\textbf{0.435}&\textbf{0.518}&\textbf{176.1}&\textbf{0.386}&\textbf{0.457}&\textbf{282.9}\\
    \hline
    \multirow{2}{*}{5\%} & RREA & 0.590&0.683&56.7&0.610&0.708&23.9&0.550&0.647&66.0\\
     & EMEA & \textbf{0.680}&\textbf{0.751}&\textbf{51.1}&\textbf{0.703}&\textbf{0.778}&\textbf{19.2}&\textbf{0.641}&\textbf{0.716}&\textbf{53.3}\\
    \hline
    \multirow{2}{*}{10\%} & RREA & 0.677&0.757&36.1&0.710&0.791&13.0&0.658&0.743&32.7\\
     & EMEA & \textbf{0.731}&\textbf{0.796}&\textbf{31.7}&\textbf{0.762}&\textbf{0.828}&\textbf{11.0}&\textbf{0.711}&\textbf{0.781}&\textbf{28.4}\\
    \hline
    \multirow{2}{*}{20\%} & RREA & 0.756&0.821&18.9&0.782&0.848&7.7&0.743&0.814&20.2\\
     & EMEA & \textbf{0.782}&\textbf{0.840}&$\textbf{18.5}$&\textbf{0.805}&\textbf{0.865}&\textbf{6.9}&\textbf{0.765}&\textbf{0.829}&$\textbf{19.3}$\\
    \hline
    \multirow{2}{*}{30\%} & RREA & 0.794&0.851&16.1&0.819&0.876&6.7&0.790&0.851&$\textbf{12.3}$\\
     & EMEA & \textbf{0.808}&\textbf{0.862}&\textbf{14.4}&\textbf{0.833}&\textbf{0.886}&$\textbf{6.6}$&\textbf{0.801}&\textbf{0.859}&12.5\\
    \hline
\end{tabular}


==> sections/tables/overall_sup_hit1.tex <==

\begin{tabular}{|c|c|c|c|c|c|c|}
    \hline
   Anno. & Method & zh\_en&fr\_en&ja\_en&dbp\_wd&dbp\_yg\\
   \hline
   \multirow{4}{*}{0.01} & PARIS & 0.001&0.016&0.002&0.190&0.451\\
    & RREA & 0.140&0.126&0.138&0.278&0.509\\
    & PRASE & 0.241&0.227&0.163&0.557&0.667\\
    & EMEA & \textbf{0.517}&\textbf{0.480}&\textbf{0.411}&\textbf{0.581}&\textbf{0.773}\\
   \hline
   \multirow{4}{*}{0.05} & PARIS & 0.221&0.281&0.226&0.537&0.608\\
    & RREA & 0.413&0.424&0.391&0.522&0.737\\
    & PRASE & 0.461&0.514&0.432&0.531&0.689\\
    & EMEA & \textbf{0.665}&\textbf{0.677}&\textbf{0.630}&\textbf{0.708}&\textbf{0.811}\\
   \hline
   \multirow{4}{*}{0.1} & PARIS & 0.414&0.473&0.395&0.623&0.640\\
    & RREA & 0.542&0.571&0.528&0.622&0.782\\
    & PRASE & 0.522&0.575&0.508&0.679&0.701\\
    & EMEA & \textbf{0.706}&\textbf{0.727}&\textbf{0.688}&\textbf{0.755}&\textbf{0.828}\\
   \hline
   \multirow{4}{*}{0.2} & PARIS & 0.532&0.584&0.511&0.690&0.676\\
    & RREA & 0.657&0.686&0.649&0.711&0.824\\
    & PRASE & 0.593&0.622&0.580&0.726&0.719\\
    & EMEA & \textbf{0.748}&\textbf{0.773}&\textbf{0.736}&\textbf{0.808}&\textbf{0.846}\\
   \hline
   \multirow{4}{*}{0.3} & PARIS & 0.589&0.628&0.577&0.739&0.696\\
    & RREA & 0.720&0.742&0.717&0.758&0.849\\
    & PRASE & 0.623&0.649&0.613&0.754&0.735\\
    & EMEA & \textbf{0.782}&\textbf{0.801}&\textbf{0.771}&\textbf{0.836}&\textbf{0.862}\\
   \hline

\end{tabular}







==> sections/tables/overall_sup_mr.tex <==

\begin{tabular}{|c|c|c|c|c|c|c|}
    \hline
   Anno. & Method & zh\_en&fr\_en&ja\_en&dbp\_wd&dbp\_yg\\
   \hline
 \multirow{2}{*}{0.01} & RREA & 652.3&366.5&684.0&317.9&64.4\\
 & EMEA & \textbf{116.4}&\textbf{72.1}&\textbf{181.3}&\textbf{72.8}&\textbf{17.6}\\
\hline
 \multirow{2}{*}{0.05} & RREA & 118.8&65.3&113.9&78.4&21.0\\
 & EMEA & \textbf{36.8}&\textbf{18.0}&\textbf{35.9}&\textbf{21.5}&\textbf{12.7}\\
\hline
 \multirow{2}{*}{0.1} & RREA & 56.9&31.3&52.6&36.2&14.0\\
 & EMEA & \textbf{27.4}&\textbf{9.7}&\textbf{24.5}&\textbf{13.4}&\textbf{9.2}\\
\hline
 \multirow{2}{*}{0.2} & RREA & 26.5&14.7&25.3&20.6&12.0\\
 & EMEA & \textbf{16.6}&\textbf{6.8}&\textbf{16.3}&\textbf{6.6}&\textbf{10.4}\\
\hline
 \multirow{2}{*}{0.3} & RREA & 16.7&9.2&14.9&14.0&6.9\\
 & EMEA & \textbf{12.6}&\textbf{5.9}&\textbf{12.6}&\textbf{7.3}&\textbf{5.8}\\
\hline

\end{tabular}







==> sections/tables/overall_sup_mrr.tex <==

\begin{tabular}{|c|c|c|c|c|c|c|}
    \hline
   Anno. & Method & zh\_en&fr\_en&ja\_en&dbp\_wd&dbp\_yg\\
   \hline
 \multirow{2}{*}{0.01} & RREA & 0.215&0.208&0.203&0.368&0.602\\
 & EMEA & \textbf{0.591}&\textbf{0.565}&\textbf{0.488}&\textbf{0.657}&\textbf{0.828}\\
\hline
 \multirow{2}{*}{0.05} & RREA & 0.518&0.539&0.496&0.616&0.803\\
 & EMEA & \textbf{0.738}&\textbf{0.757}&\textbf{0.710}&\textbf{0.778}&\textbf{0.861}\\
\hline
 \multirow{2}{*}{0.1} & RREA & 0.641&0.675&0.631&0.709&0.841\\
 & EMEA & \textbf{0.777}&\textbf{0.802}&\textbf{0.764}&\textbf{0.820}&\textbf{0.877}\\
\hline
 \multirow{2}{*}{0.2} & RREA & 0.745&0.775&0.740&0.787&0.875\\
 & EMEA & \textbf{0.815}&\textbf{0.841}&\textbf{0.807}&\textbf{0.866}&\textbf{0.891}\\
\hline
 \multirow{2}{*}{0.3} & RREA & 0.797&0.821&0.797&0.827&0.894\\
 & EMEA & \textbf{0.842}&\textbf{0.863}&\textbf{0.837}&\textbf{0.889}&\textbf{0.904}\\
\hline

\end{tabular}







==> sections/tables/sig_test_ite.tex <==


\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{Annotation} &\multicolumn{3}{c|}{zh\_en}&\multicolumn{3}{c|}{fr\_en}&\multicolumn{3}{c|}{ja\_en}\\
 & Hit@1&MRR&MR&Hit@1&MRR&MR&Hit@1&MRR&MR\\
\hline
0.01 & 0.000&0.000&0.000&0.000&0.000&0.000&0.000&0.000&0.000\\
\hline
0.05 & 0.000&0.000&0.000&0.000&0.000&0.000&0.000&0.000&0.000\\
\hline
0.1 & 0.000&0.000&0.000&0.000&0.000&0.000&0.000&0.000&0.000\\
\hline
0.2 & 0.000&0.000&0.000&0.000&0.000&0.000&0.000&0.000&0.000\\
\hline
0.3 & 0.000&0.000&0.000&0.000&0.000&0.000&0.000&0.000&0.000\\
\hline
\end{tabular}



==> sections/tables/sig_test_sup.tex <==

\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{Annotation} &\multicolumn{3}{c|}{zh\_en}&\multicolumn{3}{c|}{fr\_en}&\multicolumn{3}{c|}{ja\_en}\\
 & Hit@1&MRR&MR&Hit@1&MRR&MR&Hit@1&MRR&MR\\
\hline
0.01 & 0.000&0.000&0.000&0.000&0.000&0.000&0.000&0.000&0.000\\
\hline
0.05 & 0.000&0.000&0.000&0.000&0.000&0.000&0.000&0.000&0.000\\
\hline
0.1 & 0.000&0.000&0.000&0.000&0.000&0.000&0.000&0.000&0.000\\
\hline
0.2 & 0.000&0.000&0.000&0.000&0.000&0.000&0.000&0.000&0.000\\
\hline
0.3 & 0.000&0.000&0.000&0.000&0.000&0.000&0.000&0.000&0.000\\
\hline
\end{tabular}


